VIRD: Immersive Match Video Analysis for High-Performance Badminton Coaching

Badminton is a fast-paced sport that requires a strategic combination of spatial, temporal, and technical tactics. To gain a competitive edge at high-level competitions, badminton professionals frequently analyze match videos to gain insights and develop game strategies. However, the current process for analyzing matches is time-consuming and relies heavily on manual note-taking, due to the lack of automatic data collection and appropriate visualization tools. As a result, there is a gap in effectively analyzing matches and communicating insights among badminton coaches and players. This work proposes an end-to-end immersive match analysis pipeline designed in close collaboration with badminton professionals, including Olympic and national coaches and players. We present VIRD, a VR Bird (i.e., shuttle) immersive analysis tool, that supports interactive badminton game analysis in an immersive environment based on 3D reconstructed game views of the match video. We propose a top-down analytic workflow that allows users to seamlessly move from a high-level match overview to a detailed game view of individual rallies and shots, using situated 3D visualizations and video. We collect 3D spatial and dynamic shot data and player poses with computer vision models and visualize them in VR. Through immersive visualizations, coaches can interactively analyze situated spatial data (player positions, poses, and shot trajectories) with flexible viewpoints while navigating between shots and rallies effectively with embodied interaction. We evaluated the usefulness of VIRD with Olympic and national-level coaches and players in real matches. Results show that immersive analytics supports effective badminton match analysis with reduced context-switching costs and enhances spatial understanding with a high sense of presence.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
last modified by Bernhard Finkbeiner, July 5, 2010

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored by
the IEEE Visualization & Graphics Technical Committee (VGTC).

The only conferences that use the 'journal' document option:
- IEEE Visualization Conference (Research and Application Papers Only)
- IEEE Information Visualization Conference (Research and Application
Papers Only)

It contains 13 files:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed,
                  somewhere in the TeX search path
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
sample.eps      - an image used by the example paper
sample.pdf      - its PDF version
template-journal*.pdf    - an example proper pdf output in default
                          conference mode, with and without teaser
CypressView.eps - teaser image
CypressView.pdf - its PDF version
makefile     - makefile including bibtex compilation and proper PDF
                generation

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We
suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create
a file called 'template.pdf'. Please make sure, that its layout is
identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process
manually.  Below are a list of available options that may be passed to
make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> docs/_deprecated/1_intro_v1.tex <==
% !TEX root = ../main.tex

\firstsection{Introduction}
\maketitle

% importance of video analysis in badminton coaching and training

Professional badminton players compete at the highest level, and the outcomes of their matches are often decided by the narrowest of margins. 
Players and coaches have come to rely heavily on match analysis to identify key patterns and strategies that can be used to gain a competitive advantage against their opponents. 
As a result, match analysis is a crucial part of badminton coaching, which requires a combination of data analytics, domain expertise, 
and coaching experiences to develop useful winning strategies and training plans for the player.

% coaching
Different from training, coaching provides crucial guidance for players to develop training and playing strategies by extracting and prioritizing valuable insights from match analyses. 
The success of badminton coaching relies on several factors, including the coach's expertise, resources available to collect and analyze data, and the amount and quality of the coaching time with the player.
% 
%% challenges
% At the competitive level, coaches and players have to study the game and develop strategies against different opponents through video analysis. 
To analyze one game, a coach has to watch hundreds of rallies, each of which contains tens of shots, while jotting down notes on a piece of paper. To make things worse, to develop and confirm insights, they typically have to do this for each video from start to finish a dozen of times. This painful process requires a significant amount of time (3 to 5 times the video length) and a lot of mental effort. This in turn compresses the time coaches can spend with their players. Combining it with a lack of effective means to communicate these tactical insights to each player, we found that there is a huge demand for more efficient video analysis and coaching tool.


%However, current badminton coaching is still very manual and lacks support for iteration. 
%The current video analysis process requires repetitive video watching and manual note-taking. 
%For individual sports like badminton, coaches often have limited access to data, means of expression, and coaching time with individual players. 
%This causes a gap in video analysis and communication between coaches and players due to a lack of supporting coaching materials.

% Overview of current methods and tools for video analysis

\jui{It might make sense to have a paragraph here to contrast what existing work is doing in more qualitative ways, and then specify the gaps in these work in addressing our problems}

% Statement of the problem and research questions

In this work, 
we propose an integrated immersive analysis pipeline for badminton matches based on close collaboration with top Olympic-level badminton professionals. 
We aim to answer the following three questions from our study:
\begin{itemize}
\item What data are required for analyzing matches and developing coaching insights? 
\item What is the ideal coaching workflow for badminton video analysis and communication?
\item How to design an integrated video analysis tool to support badminton coaching for professional coaches and players?
\end{itemize}

Using computer vision (CV) techniques, 
we extract rally and shot-level data from a match video and reconstruct dynamic trajectories in 3D. 
We design a top-down approach where coaches can overview all shots in a summary view, and examine individual rally videos in a detailed view. 
Through 3D immersive visualization, coaches can interactively analyze the spatial data with visceral experiences of dynamic shots from the player's perspectives and perform video analysis with efficient playback and searching.

% WHY VR? <--- better to say it upfront than having reviewers complain why we didn't compare with 2D.
To propel the immersive
analytics in sports, we experiment the use of immersive 3D visualizations and embodied interaction in VR. 
Our case studies suggest (VR benefits for sports analytics)

% Objectives and contributions of the proposed VR tool

\jui{Another question I have is whether we can elevate the framing of the paper to include other competitive individual sports like Tennis, and then specify why and how we focus on badminton.}


Our contribution is three folds, 
(1) a formative study with Olympic-level badminton athletes to characterize current workflow and gaps in match analysis for coaching, 
(2) an end-to-end immersive video analytic tool for badminton coaching, VIRD, and (3) case studies of VIRD with high-performance badminton experts on analyzing real matches.
We concluded with research implications
for applying immersive analytics to sports coaching with automatic data collection and a human-in-the-loop analysis approach.

==> docs/_deprecated/3_background.tex <==
% !TEX root = ../main.tex

% \section{Background}

% \subsection{Badminton Match Analysis and Coaching}
% match analysis
% Professional badminton players compete at the highest level, and the outcomes of their matches are often decided by the narrowest of margins. 
% As a result, players and coaches have come to rely heavily on match analysis as a means of identifying key patterns and strategies that can be used to gain a competitive advantage against their opponents. 
% % coaching
% Different from training, coaching provides crucial guidance for players to develop training and playing strategies by extracting and prioritizing valuable insights from match analyses. 
% The success of badminton coaching relies on several factors, including the coach's expertise, resources available to collect and analyze data, and the amount and quality of the coaching time with the player.
% \jui{This paragraph seems largely overlapping with intro. Consider removing or at least shortening}

% rule: https://olympics.com/en/news/badminton-guide-how-to-play-rules-olympic-history
% A badminton match consists of the best-of-three games. 
% A game is won by the first side to win 21 points or two clear points if the score is 20-20. 
% Each point is earned by winning a rally, which involves multiple shots (strokes). 
% % The side that won the previous rally serves first in the next rally. 
% % A point is scored when the bird (shuttlecock) hits the ground in the opponent's court.
% Players change sides after each game and at the midway point of the third game, when one side reaches 11 points. 
% A break is allowed at the midpoint of each game. A typical match takes 40-50 minutes, but the duration can vary depending on the players and circumstances. \jui{the only useful thing in this paragraph seems to be the duration of a typical game. Can we just add it to the intro and remove this paragraph?}

% \subsection{CV Techniques}

% \subsubsection{Pose and shape estimation}
% Using statistical models and a top-down approach, CLIFF (Carrying Location Information in Full Frames)\cite{li-2022} performs a 3D human pose and shape estimation from a single RGB image. The first step is the detection of players. This is done using YoloV3 \cite{yolov3}, a fast and accurate model that predicts object class and bounding boxes by dividing the image into a grid of cells. Then, the prediction of the SMPL parameters from image features is done using regression-based methods. This estimation is used to obtain the human body meshes through a linear function, resulting in a complete 3D representation of the players. \jui{Why do we need these details? Isn't it just applying off-the-shelf technique? If so, we should focus on WHY we need the pose and for the implementation details, just cite the paper. Same for the trajectory reconstruction; my view is we need only a very short description of what we did there, too.}

% \section{Methodologies}
% We applied a user-centered design process to develop VIRD and involved target users (i.e., professional coaches and players) at every design stage. 
% We interviewed experts to identify the design requirements (Sec.\ref{sec:goal_task_analysis}}), 
% and iterate our design decision based on three rounds of  user testing (Sec.\ref{sec:vird}), 
% and finally, we evaluated the use of our tool in analyzing actual matches in a user study (Sec.\ref{sec:user-study}).
% Note that due to the specific domain we target, i.e., high-performance badminton coaching, our design is guided by a small number of domain experts involved in the study. While this is the nature of professional sports, we discuss the implications of conducting research with professional athletes in Sec.~\ref{sec:proathletes}.
% \jui{This is important. However, if we remove 3.1-3.2 (or combine them with intro, then we can put this at the end of the intro as well?}

==> docs/_deprecated/3_formative_v2.tex <==
% !TEX root = ../main.tex

\section{Formative Study with Olympian Coaches & Players}
\tl{WIP}
% We applied a user-centered design process to develop VIRD and involved target users (i.e., professional coaches and players) at every design stage. 
% Section \ref{sec:goal_task_analysis} presents our process of obtaining design requirements based on expert interviews. 
% Section \ref{sec:vird} presents VIRD's design based on three rounds of user testing.
% Finally, section \ref{sec:user-study} presents the evaluation of VIRD in analyzing actual matches in case studies.

% Note that due to the specific domain we target, i.e., high-performance badminton coaching, our design is guided by a small number of domain experts involved in the study. While this is the nature of professional sports, we discuss the implications of conducting research with professional athletes in Sec.~\ref{sec:proathletes}.

% \jui{unprofessional question here: should this section really be called "Design Requirement"? Doesn't seem to match what comes next... But maybe it is a field thing..}

% We interviewed 5 badminton professionals on their coaching experiences to obtain insights into gaps in their current video analysis. 
% We iterated with 3 coaches to propose an ideal match analysis workflow and conducted goal and task analysis to form design requirements. 

% \jui{One thing I think will be good to clarify here or in intro is why we have so few interviewees -- due to our focus on high level players.}

\subsection{Procedures}
\label{sec:formativestudy}
To understand current practice and identify gaps in badminton coaching, we interviewed five professional badminton players and coaches (I1-I5; M = 2, F = 3; Age:
30-40). All of them are former Olympic-level players representing Canada, Taiwan, and the US. All of them have at least 10 years of player experience and four became official coaches after their playing careers with 2 to 15 years of coaching experience.

We conducted 1-hour semi-structured interviews online to elicit the interviewee's background, overall coaching workflow, video and data usage in their coaching, and how they evaluate the player's performance in the video analysis. Finally, we asked interviewees to analyze a short match video to demonstrate their typical analysis workflow. 

All interviews were transcribed and analyzed using affinity mapping. Our analysis focused on understanding the current badminton coaching practice and identifying gaps in their match analysis workflow. 


\subsection{Findings and Discussions}
We present findings on coaching workflow, the current practice of match analysis, and the usage of videos. Finally, we highlight the pain points of performing match analysis on videos.

\subsubsection{Coaching Workflow}
% \para{Effective analysis and communication are essential for coaching, regardless of the method.}

\para{Coaching resources and styles vary widely.}
We observed coaching practices vary widely among the interviewees. 
This variation can be explained by a few variables. First, the level of resources available to a player can vary significantly depending on their level of competition, with high performers or older players typically receiving more attention. 
% 
Second, the coach-player relationship 
% (e.g., familiarity, personalities)
can impact the dynamics and ultimately the outcome of the coaching, as emphasized by a coach that \textit{``you really have to understand the individual and know how they respond to certain things''} (I2). 
% 
Third, coaches' own preference and familiarity with the available technology stack shape their coaching style. 
Some coaches use data analysis (e.g., notational analysis) to reveal errors and shot patterns (I1, I2), while others gain insights on playing styles and shot quality from match videos (I3, I4).
% Some coaches perform data analysis (i.e., notational analysis) to reveal errors and shot patterns (I1, I2), while others obtain general insights on playing styles and shot quality from the match videos (I3, I4). 
% 
Finally, the player's skill level impacts the instruction types. 
Novices receive guidance on basic tactics and pose correctness, while elite athletes focus on tactical-level instruction.
% Less experienced players will get instructions on basic tactics and pose correctness, whereas elite athletes get instructions at a tactical level.
%At lower level more instructions will be given on basic tactics and pose correctness, whereas at higher level, the instructions are given at a tactic level.

%Through coaching, players receive guidance on the areas they need to focus on to improve their game throughout their careers. However, the level of resources available to players can vary significantly depending on the level of competition.
%Coaches often have limited time to spend with lower-ranked or younger players compared to the high-performance groups.
%Particularly, the individual coach-player relationship has a huge impact on how a player can benefit from coaching. Each coach has a different style and 
%players' needs for coaching evolve as they grow and develop (I1-I5). 
%From a coach's perspective,
%\textit{``you really have to understand the individual and know how they respond to certain things''} (I2). Some coaches perform data analysis (i.e., notational analysis) to reveal errors and shot patterns (I1, I2), while others obtain general insights on playing styles and shot quality from the match videos (I4).
%Players' needs for coaching also change from basic tactics at a lower level to studying the game at a higher level. 

\para{Coaching involves a common two-step process, requiring effective analysis and communication.}
Despite the difference in coaching style, the overall coaching process includes an analysis and a communication step.
Coaches or players take notes from watching the match, analyze the notes to obtain insights, and communicate and discuss the findings together. 
% For example, the coach watches the game to synthesize insights, and discusses them with the players to develop their future game strategy, e.g., 
With more resources, coaches can share their insights with the player,
\textit{``I have to spend 30 minutes per player writing things down, and another 1 hour to review notes with them to show them here’s what happened''} (I2). 
In other cases when access to the coach is limited, 
% when less resources are available to individual players,
the players will initiate the contact and request coaching on areas to improve (I3, I5) and 
% as the access to one's coach is sometimes limited, 
may also have to help coach each other (I1, I3, I4). This practice is helpful for players to develop strategic insights towards the game, \textit{``having that coaching lens allows you to see what patterns they scope out, or how they diagnose a problem''} (I3). 
Therefore, analyzing matches for coaching is crucial for both coaches and players.
% \jui{should we point out that our users, therefore, CAN be coach and players?}

% \para{The key to effective coaching is two-way communication and collaboration.}
% Nonetheless, 
% the key to effective coaching is communication and collaboration, enabling coaches to develop personalized strategies for players. 
% % the most effective coaching builds upon communication and collaboration to develop a personalized strategy for players. 
% As one player put it, \textit{``most of the best coaches watch [the videos] with you, and point out the pattern again and again''} (I3). 




\subsubsection{Current Workflow for Match Analysis}
\label{sec:gaps}
% Based on the interview results, we identified gaps in the current coaching workflow and propose a top-down analysis approach.
To sample their current video analysis process, we asked coaches to analyze a badminton game for 10 minutes and think-aloud their observations and coaching advice. 

% \para{Current workflow.} 
\para{Coaches obtain instant insights from reviewing matches but require cross-referencing to verify the insights.}
We observed that these high-performance coaches can identify immediate insights on the opponent's playing style and weakness the first time watching the game. For example, \textit{``She's a lefty, and her stance is a little bit untraditional. She tends to lean more to her left side so she can have a big forehand''} (I3), or in another game, \textit{``The blue guy always returns with a backhand technique. I can tell that Blue guy is very confident and comfortable in his backhand''} (I2).
However, to give their player coaching advice, coaches all requested to watch more films in order to verify their observations with more complete data,
\textit{``Right there we saw all of her forehand shots were straight mostly. But don't know until we watch more''} (I3). Further analysis is required, \textit{``I’ll switch and change more into his forehand and see if he’s more aggressive or less''} (I2). 

As we found in the interviews, the current workflow is primarily a \emph{bottom-up approach}, which involves sequentially watching the game and taking notes, until some insights emerge and are then verified.


\noindent
\textbf{Gaps.} We found gaps in data collection and presentation in the current analysis workflow.
%to support match analysis for coaches. 
On the one hand, it is difficult to  observe, take notes, extract statistics, and develop strategies at the same time. Therefore, coaches have to watch films multiple times. For each watch, they focus on different aspects, one at a time, such as opponent versus their player,
% number of shots in a rally,
and winner shots versus unforced errors. They manually note down any of these findings,
\textit{``As you can tell that process is very manual and takes up a lot of time''} (I2).
On the other hand, with limited time and resources to review footage, coaches and players might choose to only look at the most important parts, which leads to incomplete analysis and potentially less effective communication. 
Coaches have to cross-reference multiple videos to make confident conclusions, 
\textit{``Is this just an outlier or some of these random matches where we didn't do well, or concrete things that we need to work on?''} (I2).
More experienced coaches might do better at this sifting process, but they might also miss important insights. 
In addition, without ample video evidence, sometimes it can be hard to convince the players of a particular finding,
% \jui{can we quote one here?}.
\textit{``The kids don’t realize that they make a lot of unforced errors. If they knew what the rate was, they'll understand it better''} (I1).
%Coaches will leverage their experiences and observations to point out the most useful and practical part to the players, but it remains challenging for them to communicate insights effectively without concrete evidence such as video.


%Because of limited resources in badminton, even at the high-performance level, coaches we interviewed have to manually annotate everything, such as the number of shots in a rally, winners and unforced errors. Besides, they focus on different aspects one at a time from watching the raw footage (e.g., opponent vs. player), leading to much time on navigating and comparing the videos with collected data. 
%On the other hand, with limited time and resources to review films, coaches and players choose to only look at the most important parts, which leads to less comprehensive analysis and less effective communication. Coaches will leverage their experiences and observations to point out the most useful and practical part to the players, but it remains challenging for them to communicate insights effectively without concrete evidence such as video.


\subsubsection{Usage of Videos in Match Analysis}
\para{Video analysis is core to coaching despite its limitations.} 
Both players and coaches analyze videos to evaluate performance and derive insights. Videos are crucial as they help players become aware of their playing technique and style, and allow players to create a mental model of other players.
% why videos
Players are often told to record their own match and watch the videos multiple times, \textit{``Most coaches recommend we watch it several times and break it down to focus on one thing at a time''} (I3). Coaches also rely on videos to communicate insights to players. \textit{``They won’t understand what I am saying unless they see it physically''} (I2).

% video analysis focus
The focus of video analysis depends on opponents and individual matches.  During the competition, they analyze 1 to 3 games about their opponent in depth to scout the opponent's overall style and occasions when errors happen (I2, I3, I4). 
Players also compare their performance in tournaments and training to track improvement. 
Specifically, they identify patterns
% extract useful information 
from selected rallies, 
such as shot types,
% (e.g., offensive or defensive)
locations, sequence, and body movement,  where
\textit{``Some rallies are more informative and impactful than others, like longer rallies or the ones that repeat every time. I would review those more in depth''} (I3). 
% Important factors in a rally include the used shot types (e.g., offensive or defensive), shot locations, sequence of shots, and change in body movement. 
Some coaches manually extract summary statistics (and spend even more time) to reveal patterns quantitatively to better communicate with the players (I1, I2), e.g., \textit{``70\% of time when you do this, you win the point.''}   

% video analysis resource
All interviewees agreed that video analysis is critical but time-consuming. \textit{``If the match is 30-40 minutes, it took 3 to 5 hours to rewatch and discuss with your coach''} (I4). Coaches found it beneficial to analyze multiple matches of their players over a period of time (I1, I2, I4).
% \textit{``Right now I have annotated one or two matches because I don’t have time to do everything. 
\textit{``If you had like 20 matches that you played for an entire year, then you have a better idea where you can dictate training''} (I1). 


When asked about the limitation of analyzing matches with videos, 
some coaches expressed that videos 
recorded by a single camera may lose fidelity on real game aspects, 
 % especially those recorded by a single camera in badminton tournaments, can lose fidelity on real game aspects, 
 such as environmental conditions (e.g., wind), shot timing (\textit{``Speed seems slower in the video''}), and player reactions (e.g., emotional cues).
% 
% Furthermore, some coaches express that videos from a single camera itself are limiting on how accurate information can be obtained from the analysis, such as court condition, player movement, shot timing and speed \jui{I don't understand this statement. Is it better to say single camera videos might alter perceptions of the game?}, \textit{``Speed seems slower in the video''}(I2). 
Some coaches found 360-degree videos useful for comparing players and their opposition, as 
\textit{``you can 
see both sides and 
% of things happen and their interaction,
% , and you can see the interaction 
like 
how the player reacts to the opponent in real-time''} (I1). Slow-motion or zoomed views also help to break down the technique and provide objective viewpoints (I1, I3), \textit{``when you're hitting the shot, you only know how it feels, but you can't see how it looks''} (I3). 


\subsection{Summary}
Even though videos are core to coaching, currently the value obtained from these videos is sub-optimal due to the limitation on coaching resources. 
Single-viewpoint videos also have limitations on the spatial perception of the real game.
Experts have developed ways to enhance the coaching workflow, such as using notational analysis to collect stats or capturing 360 videos to allow multi-angle analysis; they also leverage tools to manage videos and communicate with the players, such as YouTube and Clutch~\cite{clutch}. 
% \jui{the 360 thing seems out of place here}. 
However, there is currently no ideal solution for efficiently conducting comprehensive video analysis.

==> docs/_deprecated/3_formative_v3.tex <==
% !TEX root = ../main.tex

\section{Formative Study with Olympian Coaches & Players \zt{WIP}}
% We applied a user-centered design process to develop VIRD and involved target users (i.e., professional coaches and players) at every design stage. 
% Section \ref{sec:goal_task_analysis} presents our process of obtaining design requirements based on expert interviews. 
% Section \ref{sec:vird} presents VIRD's design based on three rounds of user testing.
% Finally, section \ref{sec:user-study} presents the evaluation of VIRD in analyzing actual matches in case studies.

% Note that due to the specific domain we target, i.e., high-performance badminton coaching, our design is guided by a small number of domain experts involved in the study. While this is the nature of professional sports, we discuss the implications of conducting research with professional athletes in Sec.~\ref{sec:proathletes}.

% \jui{unprofessional question here: should this section really be called "Design Requirement"? Doesn't seem to match what comes next... But maybe it is a field thing..}

% We interviewed 5 badminton professionals on their coaching experiences to obtain insights into gaps in their current video analysis. 
% We iterated with 3 coaches to propose an ideal match analysis workflow and conducted goal and task analysis to form design requirements. 

% \jui{One thing I think will be good to clarify here or in intro is why we have so few interviewees -- due to our focus on high level players.}

\subsection{Procedures}
\label{sec:formativestudy}
To understand current practice and identify gaps in badminton coaching, we interviewed five professional badminton players and coaches (I1-I5; M = 2, F = 3; Age:
30-40). All of them are former Olympic-level players representing Canada, Taiwan, and the US. All of them have at least 10 years of player experience and four became official coaches after their playing careers with 2 to 15 years of coaching experience.

We conducted 1-hour semi-structured interviews online to elicit the interviewee's background, overall coaching workflow, video and data usage in their coaching, and how they evaluate the player's performance in the video analysis. Finally, we asked interviewees to analyze a short match video to demonstrate their typical analysis workflow. 

All interviews were transcribed and analyzed using affinity mapping. Our analysis focused on understanding the current badminton coaching practice and identifying gaps in their match analysis workflow. 


\subsection{Findings and Discussions}
Overall, we observed coaching practices vary widely among the interviewees. 
% This variation can be explained by a few variables. First, the level of resources available to a player can vary significantly depending on their level of competition, with high performers or older players typically receiving more attention. 
% Second, the coach-player relationship 
% can impact the dynamics and ultimately the outcome of the coaching, as emphasized by a coach that \textit{``you really have to understand the individual and know how they respond to certain things''} (I2). 
% Third, coaches' own preference and familiarity with the available technology stack shape their coaching style. 
% Some coaches use data analysis (e.g., notational analysis) to reveal errors and shot patterns (I1, I2), while others gain insights on playing styles and shot quality from match videos (I3, I4).
% Finally, the player's skill level impacts the instruction types. 
% Novices receive guidance on basic tactics and pose correctness, while elite athletes focus on tactical-level instruction.
Despite the difference in coaching style, 
the coaching process typically involves two steps: analysis and communication.
Coaches and players watch matches, take notes, analyze them for insights, and discuss their findings. 
With more resources, coaches can share their insights with players, although this requires a significant time investment (I2). 
 % With more resources, coaches can share their insights with the player,
% \textit{``I have to spend 30 minutes per player writing things down, and another 1 hour to review notes with them to show them here’s what happened''} (I2). 
Alternatively, in cases where access to a coach is limited, 
players may initiate contact and request coaching on areas to improve (I3, I5)
or help coach each other (I1, I3, I4). 
% In other cases when access to the coach is limited, 
% the players will initiate the contact and request coaching on areas to improve (I3, I5) and 
% may also have to help coach each other (I1, I3, I4). 
% This practice is helpful for players to develop strategic insights towards the game, \textit{``having that coaching lens allows you to see what patterns they scope out, or how they diagnose a problem''} (I3). 
This practice is useful for developing strategic insights towards the game. 
Therefore, analyzing matches for coaching is crucial for both coaches and players.

In this work, we focus on the analysis step of badminton coaching
and summarized the current practice and pain points in match analysis.


% To sample their current video analysis process, we asked coaches to analyze a badminton game for 10 minutes and think-aloud their observations and coaching advice. 
\subsubsection{Current Bottom-Up Workflow is Time-Consuming}
\label{sec:gaps}
We observed that the coaches we interviewed followed a \emph{bottom-up} approach to generate their insights. 
They began by scanning videos to catch insights into the opponent's playing style and weaknesses. 
For example, during video scanning, I3 immediately noticed that \emph{``She's a lefty ... [so] She tends to lean more to her left side for a big forehand.''} 
Once they formed an insight hypothesis, they watched more videos to search for similar patterns and verify their observations. 
I3 explained, \emph{`` ... we saw all of her forehand shots were straight mostly, but don't know until we watch more.''} 
In summary, coaches repeatedly watched games until insights emerged, then re-watched the games to collect more evidence. 
However, this workflow is significantly time-consuming,
\zt{I feel we need a sentence to transit to the top-down workflow. maybe quote ``Overview first, details on demand''}
leading us to the first design goal:

\begin{quote}
\textbf{G1. Providing a top-down analysis workflow.} 
\zt{@Tica, plz refine and flesh out this a bit}
Summary data enables an immediate overview of the match and support effective exploration to discover region-of-interest for analysis. 
Per coaches' feedback, essential metadata include scores, rally count, match duration, errors and winners count, and length of each rally. 
\end{quote}

% Further analysis is required, \textit{``I’ll switch and change more into his forehand and see if he’s more aggressive or less''} (I2). 

% (I3), or in another game, \textit{``The blue guy always returns with a backhand technique. I can tell that Blue guy is very confident and comfortable in his backhand''} (I2).

% \para{Coaches obtain instant insights from reviewing matches but require cross-referencing to verify the insights.}
% We observed that these high-performance coaches can identify immediate insights  the first time watching the game. 
% However, to give their player coaching advice, coaches all 

\subsubsection{Collecting Data from Videos is Tedious}
Both players and coaches analyze videos to evaluate performance and derive insights. Videos are crucial as they help players become aware of their playing technique and style, and allow players to create a mental model of other players.
% why videos
Players are often told to record their own match and watch the videos multiple times, \textit{``Most coaches recommend we watch it several times and break it down to focus on one thing at a time''} (I3). Coaches also rely on videos to communicate insights to players. \textit{``They won’t understand what I am saying unless they see it physically''} (I2).

% video analysis resource
All interviewees agreed that video analysis is critical but time-consuming. \textit{``If the match is 30-40 minutes, it took 3 to 5 hours to rewatch and discuss with your coach''} (I4). Coaches found it beneficial to analyze multiple matches of their players over a period of time (I1, I2, I4).
\textit{``If you had like 20 matches that you played for an entire year, then you have a better idea where you can dictate training''} (I1). 


%% collecting data from video
\zt{need auto-extraction}
On the one hand, it is difficult to  observe, take notes, extract statistics, and develop strategies at the same time. Therefore, coaches have to watch films multiple times. For each watch, they focus on different aspects, one at a time, such as opponent versus their player,
and winner shots versus unforced errors. They manually note down any of these findings,
\textit{``As you can tell that process is very manual and takes up a lot of time''} (I2).
On the other hand, with limited time and resources to review footage, coaches and players might choose to only look at the most important parts, which leads to incomplete analysis and potentially less effective communication. 

% video analysis focus
The focus of video analysis depends on opponents and individual matches.  
During the competition, they analyze 1 to 3 games about their opponent in depth to scout the opponent's overall style and occasions when errors happen (I2, I3, I4). 
Players also compare their performance in tournaments and training to track improvement. 
Specifically, they identify patterns from selected rallies, such as shot types,
locations, sequence, and body movement,  where
\textit{``Some rallies are more informative and impactful than others, like longer rallies or the ones that repeat every time. I would review those more in depth''} (I3). 
Some coaches manually extract summary statistics (and spend even more time) to reveal patterns quantitatively to better communicate with the players (I1, I2), e.g., \textit{``70\% of time when you do this, you win the point.''}   

\subsection{Presenting Insights with Videos is Necessary}
%% presenting data with video
\zt{need presenting insights with videos}
In addition, without ample video evidence, sometimes it can be hard to convince the players of a particular finding,
\textit{``The kids don’t realize that they make a lot of unforced errors. If they knew what the rate was, they'll understand it better''} (I1).

Coaches have to cross-reference multiple videos to make confident conclusions, 
\textit{``Is this just an outlier or some of these random matches where we didn't do well, or concrete things that we need to work on?''} (I2).
More experienced coaches might do better at this sifting process, but they might also miss important insights. 


\textbf{G2. Integrate static data and video to support comprehensive analysis.} 
\zt{merge abstract data with the physical context} 
Even though summary data can help coaches identify patterns in the game, it is still important to investigate the actual game moments in the video to verify observations and analyze the root cause, as well as present the insights to players. 
Providing an easy transition between statistics and videos is thus crucial to support iterative analytical reasoning and communication.


\subsubsection{2D displays are insufficient}
% \para{Video analysis is core to coaching despite its limitations.} 

\zt{3D reconstruction}
When asked about the limitation of analyzing matches with videos, 
some coaches expressed that videos 
recorded by a single camera may lose fidelity on real game aspects, 
such as environmental conditions (e.g., wind), shot timing (\textit{``Speed seems slower in the video''}), and player reactions (e.g., emotional cues).
Some coaches found 360-degree videos useful for comparing players and their opposition, as 
\textit{``you can see both sides and like 
how the player reacts to the opponent in real-time''} (I1). Slow-motion or zoomed views also help to break down the technique and provide objective viewpoints (I1, I3), \textit{``when you're hitting the shot, you only know how it feels, but you can't see how it looks''} (I3). 

%%%%%%%%%%%%%%%%%%%%%%%%%%G1 - G3
% Based on user interviews, we identified that high-performance badminton coaches and players perform match analysis to reveal the strengths and weaknesses of the opponent/player and develop playing or training strategies. However, data collection and presentation gaps exist in their current analysis workflow.

% To support these coaches and players in analyzing matches and communicating insights effectively, we characterized three design goals to support an ideal analytic workflow.


% % 
% % Since match analysis requires investigation into action details like dynamic movement and player pose, it is important to allow easy reference to the actual video when providing statistics. \jui{the conclusion is ok, but the reasoning seems weak -- what part of the analysis requires action details? Did we support this statement in the formative studies? We need to explain things better here and potentially re-word G2.}
% \textbf{G3. Visualize spatial and temporal data within context.} 3D data (e.g., shot trajectory or player position) should be represented within the appropriate context to support an accurate interpretation of their spatial and temporal attributes, such as speed and timing. In addition, our visualizations should support experts analyzing from flexible viewpoints to allow accurate spatial perception and objective perspectives. 
% % \jui{same here. I feel like this is the right goal, but insufficiently supported in the studies we presented so far. Need to adjust the formative studies part to accommodate this statement.}

% From the user's perspective, we abstract five visualization tasks that are performed throughout the match analysis. 


\subsection{Summary}
Even though videos are core to coaching, currently the value obtained from these videos is sub-optimal due to the limitation on coaching resources. 
Single-viewpoint videos also have limitations on the spatial perception of the real game.
Experts have developed ways to enhance the coaching workflow, such as using notational analysis to collect stats or capturing 360 videos to allow multi-angle analysis; they also leverage tools to manage videos and communicate with the players, such as YouTube and Clutch~\cite{clutch}. 
% \jui{the 360 thing seems out of place here}. 
However, there is currently no ideal solution for efficiently conducting comprehensive video analysis.


\noindent
\textbf{T1.  Break down a match into rallies.}
A user first needs a breakdown of the match to obtain necessary metadata (e.g., winning rallies, game length) and easy access to the rallies of interest. \textit{Gap: There is currently no direct way to navigate to or filter rallies based on game information.}

\noindent
\textbf{T2.  Extract statistics from videos at rally and shot levels.}
The user explores summary data, such as rally lengths and shot locations, to obtain an overall impression of the game (e.g., playing style, rhythm). The statistics allow them to obtain an overview, which leads to identifying specific patterns in the next steps. \textit{Gap: Currently, users have to watch the entire video to annotate and collect this data.}

\noindent
\textbf{T3.  Identify patterns of winner \& error shots.}
% The user then focuses on rallies that led to winner and error shots to derive insights based on summarizing and comparing the identified patterns. 
The user then focuses on analyzing winner and error shots to derive insights. 
Necessary aspects to consider include spatial and temporal analysis of shot trajectories and player poses, and their comparison with the summarized attributes such as shot types and distributions. \textit{Gap: Shots and rallies are not categorized and have to be found manually.  
Spatial and dynamic data are not presented in-situ and in 3-dimensional perspectives. }

\noindent
\textbf{T4.  Investigate game details of a rally.}
% \jui{I think they look at more than just the pose etc in the video. Should we broaden this task to obtaining more detailed information in the video but missing from our higher-level summary and statistics.}
Once some patterns are observed, the user dives into the respective game moments of the rally to examine game details that are missing from the summary statistics, such as player movement and strategy, to contemplate deeper into the cause of the performance. 
% \jui{In general, we should proabably lay the foundation better in earlier sections on answering: why is video important and what is missing from our reconstruction}
\textit{Gap: Navigating and replaying specific game moments in the video is tedious, which causes high mental load to compare summary statistics with game details. 
In addition, interpreting dynamic shots and player movement is constrained by the video angle.}
% \textit{Gap: Interpretation of the spatial and temporal aspects is constrained by the video angle.}
% \jui{not sure if this is the right gap}

\noindent
\textbf{T5.  Generate and verify insights across rallies.} Before concluding  coaching advice, the user cross-references other rallies with similar or contrasting patterns to update and verify insights. \textit{Gap: It is time-consuming to compare and organize video clips to support insights.}



==> docs/_deprecated/3_formative_v4.tex <==
% !TEX root = ../main.tex

\section{Formative Study with Olympian Coaches & Players \zt{WIP}}
% We applied a user-centered design process to develop VIRD and involved target users (i.e., professional coaches and players) at every design stage. 
% Section \ref{sec:goal_task_analysis} presents our process of obtaining design requirements based on expert interviews. 
% Section \ref{sec:vird} presents VIRD's design based on three rounds of user testing.
% Finally, section \ref{sec:user-study} presents the evaluation of VIRD in analyzing actual matches in case studies.

% Note that due to the specific domain we target, i.e., high-performance badminton coaching, our design is guided by a small number of domain experts involved in the study. While this is the nature of professional sports, we discuss the implications of conducting research with professional athletes in Sec.~\ref{sec:proathletes}.

% \jui{unprofessional question here: should this section really be called "Design Requirement"? Doesn't seem to match what comes next... But maybe it is a field thing..}

% We interviewed 5 badminton professionals on their coaching experiences to obtain insights into gaps in their current video analysis. 
% We iterated with 3 coaches to propose an ideal match analysis workflow and conducted goal and task analysis to form design requirements. 

% \jui{One thing I think will be good to clarify here or in intro is why we have so few interviewees -- due to our focus on high level players.}

\subsection{Procedures}
\label{sec:formativestudy}
To understand current practice and identify gaps in badminton coaching, we interviewed five professional badminton players and coaches (I1-I5; M = 2, F = 3; Age:
30-40). All of them are former Olympic-level players representing Canada, Taiwan, and the US. All of them have at least 10 years of player experience and four became official coaches after their playing careers with 2 to 15 years of coaching experience.

We conducted 1-hour semi-structured interviews online to elicit the interviewee's background, overall coaching workflow, video and data usage in their coaching, and how they evaluate the player's performance in the video analysis. Finally, we asked interviewees to analyze a short match video to demonstrate their typical analysis workflow. 

All interviews were transcribed and analyzed using affinity mapping. Our analysis focused on understanding the current badminton coaching practice and identifying gaps in their match analysis workflow. 


\subsection{Findings and Discussions}
Overall, we observed coaching practices vary widely among the interviewees. 
\zt{common points: 1) two steps, 2) videos}
% This variation can be explained by a few variables. First, the level of resources available to a player can vary significantly depending on their level of competition, with high performers or older players typically receiving more attention. 
% Second, the coach-player relationship 
% can impact the dynamics and ultimately the outcome of the coaching, as emphasized by a coach that \textit{``you really have to understand the individual and know how they respond to certain things''} (I2). 
% Third, coaches' own preference and familiarity with the available technology stack shape their coaching style. 
% Some coaches use data analysis (e.g., notational analysis) to reveal errors and shot patterns (I1, I2), while others gain insights on playing styles and shot quality from match videos (I3, I4).
% Finally, the player's skill level impacts the instruction types. 
% Novices receive guidance on basic tactics and pose correctness, while elite athletes focus on tactical-level instruction.
Despite the difference in coaching style, 
the coaching process typically involves two steps: analysis and communication.
Coaches and players watch matches, take notes, analyze them for insights, and discuss their findings. 
With more resources, coaches can share their insights with players, although this requires a significant time investment (I2). 
Alternatively, in cases where access to a coach is limited, 
players may initiate contact and request coaching on areas to improve (I3, I5)
or help coach each other (I1, I3, I4). 
This practice is useful for developing strategic insights towards the game. 
Therefore, analyzing matches for coaching is crucial for both coaches and players.

Both players and coaches analyze videos to evaluate performance and derive insights. 
Videos are crucial as they help players become aware of their playing technique and style, 
and allow players to create a mental model of other players.
% why videos
Players are often told to record their own match and watch the videos multiple times, \textit{``Most coaches recommend we watch it several times and break it down to focus on one thing at a time''} (I3). 
Coaches also rely on videos to communicate insights to players. 
\textit{``They won’t understand what I am saying unless they see it physically''} (I2).

% video analysis is tedious
All interviewees agreed that video analysis is critical but time-consuming. 
\textit{``If the match is 30-40 minutes, it took 3 to 5 hours to rewatch and discuss with your coach''} (I4). 
Coaches found it beneficial to analyze multiple matches of their players over a period of time (I1, I2, I4).
\textit{``If you had like 20 matches that you played for an entire year, then you have a better idea where you can dictate training''} (I1). 


In this work, we focus on the analysis step of badminton coaching
and summarized the current practice and pain points in match analysis.

\subsubsection{Current Bottom-Up Workflow is Time-Consuming}
\label{sec:gaps}
We observed that the coaches we interviewed followed a \emph{bottom-up} approach to generate their insights. 
They began by scanning videos to catch insights into the opponent's playing style and weaknesses. 
For example, during video scanning, I3 immediately noticed that \emph{``She's a lefty ... [so] She tends to lean more to her left side for a big forehand.''} 
Once they formed an insight hypothesis, they watched more videos to search for similar patterns and verify their observations. 
I3 explained, \emph{`` ... we saw all of her forehand shots were straight mostly, but don't know until we watch more.''} 
In summary, coaches repeatedly watched games until insights emerged, then re-watched the games to collect more evidence. 
However, this workflow is significantly time-consuming,
\zt{I feel we need a sentence to transit to the top-down workflow. maybe quote ``Overview first, details on demand''}
leading us to the first design goal:

\begin{quote}
\textbf{G1. Providing a top-down analysis workflow.} 
\zt{@Tica, plz refine and flesh out this a bit}
Summary data enables an immediate overview of the match and support effective exploration to discover region-of-interest for analysis. 
Per coaches' feedback, essential metadata include scores, rally count, match duration, errors and winners count, and length of each rally. 
\end{quote}

\subsubsection{Collecting Data from Videos is Tedious}
During the current workflow,
coaches manually collect summary statistics (and spend even more time) to reveal patterns quantitatively to better communicate with the players (I1, I2), e.g., \textit{``70\% of time when you do this, you win the point.''}
Players also compare their performance in tournaments and training 
by counting patterns from selected rallies, such as shot types, locations, sequence, and body movement.
However, it is difficult to pay attention to multiple metrics and patterns simultaneously.
Therefore, coaches and players have to watch films multiple times and
focus on different aspects, one at a time, such as opponent versus their player,
and winner shots versus unforced errors. 
Such a manual process \emph{``takes up a lot of time''} (I2).
Consequently,
coaches and players might choose to only look at the most important parts, 
which leads to incomplete analysis and potentially less effective communication. 
Therefore, it is essential to incorporate the design goal that

\begin{quote}
    \textbf{G2. Collecting data from videos automatically.}
    \zt{@Tica, add one more goal here to talk about auto data collection.}
\end{quote}

% with limited time and resources to review footage, 
% They manually note down any of these findings, 
% \textit{``As you can tell that process is very manual and 
% The focus of video analysis depends on opponents and individual matches.  
% During the competition, they analyze 1 to 3 games about their opponent in depth to scout the opponent's overall style and occasions when errors happen (I2, I3, I4). 

% \textit{``Some rallies are more informative and impactful than others, like longer rallies or the ones that repeat every time. I would review those more in depth''} (I3). 

%% collecting data from video
% On the one hand, it is difficult to observe, take notes, extract statistics, and develop strategies simultaneously. 
% For each watch, they 

% video analysis focus



\subsection{Presenting Insights with Videos is Necessary}
%% presenting data with video
\zt{need presenting insights with videos}
In addition, without ample video evidence, sometimes it can be hard to convince the players of a particular finding,
\textit{``The kids don’t realize that they make a lot of unforced errors. If they knew what the rate was, they'll understand it better''} (I1).

Coaches have to cross-reference multiple videos to make confident conclusions, 
\textit{``Is this just an outlier or some of these random matches where we didn't do well, or concrete things that we need to work on?''} (I2).
More experienced coaches might do better at this sifting process, but they might also miss important insights. 


\textbf{G2. Integrate static data and video to support comprehensive analysis.} 
\zt{merge abstract data with the physical context} 
Even though summary data can help coaches identify patterns in the game, it is still important to investigate the actual game moments in the video to verify observations and analyze the root cause, as well as present the insights to players. 
Providing an easy transition between statistics and videos is thus crucial to support iterative analytical reasoning and communication.


\subsubsection{2D displays are insufficient}
% \para{Video analysis is core to coaching despite its limitations.} 

\zt{3D reconstruction}
When asked about the limitation of analyzing matches with videos, 
some coaches expressed that videos 
recorded by a single camera may lose fidelity on real game aspects, 
such as environmental conditions (e.g., wind), shot timing (\textit{``Speed seems slower in the video''}), and player reactions (e.g., emotional cues).
Some coaches found 360-degree videos useful for comparing players and their opposition, as 
\textit{``you can see both sides and like 
how the player reacts to the opponent in real-time''} (I1). Slow-motion or zoomed views also help to break down the technique and provide objective viewpoints (I1, I3), \textit{``when you're hitting the shot, you only know how it feels, but you can't see how it looks''} (I3). 


\textbf{G3. Visualize spatial and temporal data within context.} 3D data (e.g., shot trajectory or player position) should be represented within the appropriate context to support an accurate interpretation of their spatial and temporal attributes, such as speed and timing. In addition, our visualizations should support experts analyzing from flexible viewpoints to allow accurate spatial perception and objective perspectives. 

%%%%%%%%%%%%%%%%%%%%%%%%%%G1 - G3
% Based on user interviews, we identified that high-performance badminton coaches and players perform match analysis to reveal the strengths and weaknesses of the opponent/player and develop playing or training strategies. However, data collection and presentation gaps exist in their current analysis workflow.

% To support these coaches and players in analyzing matches and communicating insights effectively, we characterized three design goals to support an ideal analytic workflow.


% % 
% % Since match analysis requires investigation into action details like dynamic movement and player pose, it is important to allow easy reference to the actual video when providing statistics. \jui{the conclusion is ok, but the reasoning seems weak -- what part of the analysis requires action details? Did we support this statement in the formative studies? We need to explain things better here and potentially re-word G2.}

% % \jui{same here. I feel like this is the right goal, but insufficiently supported in the studies we presented so far. Need to adjust the formative studies part to accommodate this statement.}

% From the user's perspective, we abstract five visualization tasks that are performed throughout the match analysis. 


\subsection{Summary}
Even though videos are core to coaching, currently the value obtained from these videos is sub-optimal due to the limitation on coaching resources. 
Single-viewpoint videos also have limitations on the spatial perception of the real game.
Experts have developed ways to enhance the coaching workflow, such as using notational analysis to collect stats or capturing 360 videos to allow multi-angle analysis; they also leverage tools to manage videos and communicate with the players, such as YouTube and Clutch~\cite{clutch}. 
% \jui{the 360 thing seems out of place here}. 
However, there is currently no ideal solution for efficiently conducting comprehensive video analysis.


\noindent
\textbf{T1.  Break down a match into rallies.}
A user first needs a breakdown of the match to obtain necessary metadata (e.g., winning rallies, game length) and easy access to the rallies of interest. \textit{Gap: There is currently no direct way to navigate to or filter rallies based on game information.}

\noindent
\textbf{T2.  Extract statistics from videos at rally and shot levels.}
The user explores summary data, such as rally lengths and shot locations, to obtain an overall impression of the game (e.g., playing style, rhythm). The statistics allow them to obtain an overview, which leads to identifying specific patterns in the next steps. \textit{Gap: Currently, users have to watch the entire video to annotate and collect this data.}

\noindent
\textbf{T3.  Identify patterns of winner \& error shots.}
% The user then focuses on rallies that led to winner and error shots to derive insights based on summarizing and comparing the identified patterns. 
The user then focuses on analyzing winner and error shots to derive insights. 
Necessary aspects to consider include spatial and temporal analysis of shot trajectories and player poses, and their comparison with the summarized attributes such as shot types and distributions. \textit{Gap: Shots and rallies are not categorized and have to be found manually.  
Spatial and dynamic data are not presented in-situ and in 3-dimensional perspectives. }

\noindent
\textbf{T4.  Investigate game details of a rally.}
% \jui{I think they look at more than just the pose etc in the video. Should we broaden this task to obtaining more detailed information in the video but missing from our higher-level summary and statistics.}
Once some patterns are observed, the user dives into the respective game moments of the rally to examine game details that are missing from the summary statistics, such as player movement and strategy, to contemplate deeper into the cause of the performance. 
% \jui{In general, we should proabably lay the foundation better in earlier sections on answering: why is video important and what is missing from our reconstruction}
\textit{Gap: Navigating and replaying specific game moments in the video is tedious, which causes high mental load to compare summary statistics with game details. 
In addition, interpreting dynamic shots and player movement is constrained by the video angle.}
% \textit{Gap: Interpretation of the spatial and temporal aspects is constrained by the video angle.}
% \jui{not sure if this is the right gap}

\noindent
\textbf{T5.  Generate and verify insights across rallies.} Before concluding  coaching advice, the user cross-references other rallies with similar or contrasting patterns to update and verify insights. \textit{Gap: It is time-consuming to compare and organize video clips to support insights.}



==> docs/_deprecated/5_VIRD_v1.tex <==
% !TEX root = ../main.tex




% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=\linewidth]{images/VIRD.png}
%     \vspace{-4mm}
%     \caption{VIRD components and interaction. (a) and (b) provide match overview and allow users to examine and filter rallies listed in (c) based on game and shot details. Static immersive visualizations of 3D shot data are shown in (d), whereas dynamic game views are displayed with (e) and (f). VIRD offers embodied interaction with flexible viewpoints in VR, and support top-down analysis workflow from linking shot to rally.
%     } 
%     \label{fig:VIRD}
%     \vspace{-4mm}
% \end{figure*}


% Using Shot Filter, the user selected \textit{Top}’s shots, and saw \textit{Top} has 10 errors out of 21 points she lost \textbf{(T2)}. He then selected Errors to focus on those 10 rallies ended with an error shot by \textit{Top}. Seeing the distribution of these error shots on the Heat Map, the user found 70\% of the error shots were from the middle, and could tell that these were defensive shots from seeing the shot trajectories and video previews on the virtual court \textbf{(T3)}. The user further selected a rally from the Rally Menu among all the 10 error shot rallies and examined the player movement and the sequence that led to the error shot \textbf{(T4)}. The user watched several rallies and concluded that \textit{Top} needs to practice her defensive shots on the backhand side  \textbf{(T5)}.

\section{VIRD - \underline{V}R B\underline{ird} Video Analysis Tool}
\label{sec:vird}
Based on the identified goals and tasks, we designed VIRD, an immersive video analysis platform for high-performance badminton coaching. Targeting professional badminton coaches and players, VIRD features a top-down analysis approach and supports an integrated data and video analysis workflow based on CV-based data collection and a 3D interactive environment in VR. The designs were iterated  based on expert feedback from three coaches.
% 
The code for VIRD is open-source\footnote{The code for VIRD will be made available at https://to-be-open.github.io}.

% We first described the data preprocessing techniques, the design of VIRD, and the  design iteration with experts.




\subsection{Top-Down Analysis Workflow} 
 To address G1, we designed a \emph{top-down analysis approach} and verified it with two coaches (I1 and I2) in a follow-up interview.
% 
 The top-down user flow contains the following four steps: First, users find rallies of interest based on summary statistics (\textbf{T1, T2}). Second, they compare and analyze the filtered rallies to derive insights (\textbf{T3, T4}). Third, they investigate game details to verify insights (\textbf{T5}). Finally, they examine similar patterns across rallies to conclude insights (\textbf{T6}).

 
We tested the proposed workflow
by gathering coaches' feedback on a hypothetical top-down analysis workflow for examining a lost game. 

\scriptsize
\begin{adjustwidth}{0.5cm}{0.5cm}
Initially, the user reviews the game summary to form an impression of the match. 
 Observing a tight score of 17 (\textit{Player A}) to 21 (\textit{Player B}), the user chooses to analyze the 21 rallies where \textit{Player A} lost points (\textbf{T1}). 
%
They find 10 errors among the 21 lost points and focus their analysis on those 10 rallies ending in error shots (\textbf{T2}). 
%
On the rally level, the user finds that 6 out of 10 error rallies are short and towards the end of the game (\textbf{T3}).
Examining the heat map and shot trajectories, the user notes that 70\% are from the middle, 
and identifies them as defensive shots (\textbf{T4}). 
%
The user selects a short rally (\textbf{T5}) to study player movement and the sequence leading to the error shot. 
After watching multiple error rallies  (\textbf{T6}), the user concludes that \textit{Player A} needs to improve defensive shots on the backhand side and physical fitness.
\end{adjustwidth}

\normalsize
Both coaches agreed that this workflow is precisely what they need. \textit{``We're manually doing that because currently I won't know where exactly to go back in the video to see all the unforced errors''} (I2). 



\subsection{Computer Vision Data Preprocessing}
\label{sec:data_preprocessing}
To address G2, we applied state-of-the-art computer vision (CV) models to automate the data collection from videos.
We developed a semi-automatic data preprocessing pipeline for monocular match videos, which includes manual game breakdown, shot classification algorithms, and automatic 3D shot and player reconstruction.
% 
Based on task abstraction, three types of data must be extracted from a match video.


\para{1) Game and Rally Summary} are automatically computed based on manual annotation and output from CV models:

\begin{itemize}
    \item \emph{Rally Breakdown}: 
    To obtain a game summary, player scores and average rally statistics are required. Therefore, each game needs to be split by rallies. 
    We manually annotated the time ranges (start and end), player who serves, and the winning side of all rallies from the match video. Our algorithm then derives score and game information based on the rally breakdown.

    \item \emph{Shot Breakdown}: 
    To obtain a rally summary, the duration of each rally and shot count are required. 
    We obtain the timestamps and the hitter of each shot from running MonoTrack~\cite{liu-2022} with minor manual clean-up.
\end{itemize}



\para{2) 3D Spatial Data} are automatically reconstructed from CV models.
\begin{itemize}
    \item \emph{3D Shot Trajectory}: 
    We automatically reconstructed 3D trajectories and velocities for all shots from running MonoTrack~\cite{liu-2022}.

    \item \emph{3D Player Model}: 
    We used MonoTrack~\cite{liu-2022} to estimate  court and player positions, and CLIFF~\cite{li-2022} to predict smooth 3D player poses from videos. This combination allows for the reconstruction of 3D player models.
\end{itemize}

\para{3) Shot Statistics} are automatically derived from the 3D spatial data. 
\jui{I think if we can show some helpful illustrations for these derived statistics, it can be useful} 
\begin{itemize}
    \item \emph{Shot Tendency}: 
    To detect whether a shot leading to a point is a winner or an unforced error (as described in Shot Outcome), we first classified the shot tendency by approximating the shuttle’s velocity vector when it passes the net: the tendency is defensive when the vector is going upward (away from the ground), and offensive if opposite. This classification is derived from expert input in the formative study.
% \jui{this is motivated by Toby's need right? Should we say this (if not here, then somewhere)?}
% The velocity information is obtained from running MonoTrack~\cite{liu-2022}.

    \item \emph{Shot Outcome}:
% \jui{There are two problems here: 1) the writing makes it confusing what is shot tendency and what is classification. One way to separate them is: tendency is the attempt of the shot, and the "classification" is the outcome based on this attempt. I will clarify these two paragraphs more. 2) "classification" might not be the right choice. When I read "shot classification", I immediately think of the types of the shot, like "clears", "drives", "net drops", "smashes" etc.}
    Our algorithm categorizes shots as winners, errors, or normal shots to calculate the winner and error shot counts.
    A rally ends with a winner by the scorer or an error by the point loser.
    If the last shot is offensive by the scorer, it's a winner; if defensive by the point loser, the penultimate shot is the winner. Conversely, if the last shot is offensive by the point loser, it's an error; if defensive by the scorer, the penultimate shot is an error. All others are normal shots.
% % winner
% If the final shot is an offensive shot hit by the scorer, then it is labeled as a winner for the scorer.
% If the final shot is a defensive shot hit by the point loser, then the second last shot is a winner for the scorer.
% % error
% Conversely, if the final shot is an offensive shot hit by the point loser, then it is labeled as an error; if it is a defensive shot hit by the scorer, then the second last shot is labeled as an error by the point loser.

    \item \emph{Shot Distribution}:
    From the formative study, coaches use shot locations to classify shots into six areas on the court, including front/middle/back on the left and right sides. 
    To compute the shot distribution, 
    our algorithm projects each shot's start (from) and endpoint (to) onto the court to decide shot locations.

% Our algorithm projects each shot's start and end point onto the court\jui{it might not be clear to the reader why the projection is needed. Explain it slightly more.}, and computes the shot distribution across seven court areas on each side, including front/middle/back on the left and right sides or out-of-bound.

\end{itemize}

\vspace{1mm}
\noindent
Overall, our data preprocessing pipeline is largely automated. 
Except for rally breakdown and winner/server annotation, all other data are obtained through automatic algorithms. 
% \jui{the winners and serves are also annotated. Also, I might supplement that this limitation can be addressed in cv but is out of scope for this paper}.
The manual annotation takes up roughly half of the video duration (e.g., 30 minutes for labeling a 1-hour video).
While our method is not entirely automatic, we anticipate that CV techniques may be able to address these manual annotations in the future, though they are beyond the scope of our current study.

% In a first step, match videos need to be parsed to extract match-level and rally-level statistics and spatial data. We build on previous work in computer vision to assemble a semi-automatic data processing pipeline.
% Specifically, we use MonoTrack~\cite{liu-2022} to predict court and player positions, detect shots, and reconstruct 3D trajectories from monocular badminton videos for a rally; and we use CLIFF~\cite{li-2022} to predict smooth 3D player poses from monocular videos. 
% In addition, we manually annotate rallies to extract detailed time ranges and label the winning side for each rally.
% We outline the important video-derived data we use in VIRD with a short description of how they are computed in Table~\ref{tab:data}.


% {\renewcommand{\arraystretch}{1.2}% for the vertical padding
% \begin{table}
%     \scriptsize
%     \centering
%     \caption{Preprocessed match data from the video.}
%     \label{tab:data}
%     \vspace{-1em}
%     \begin{tabularx}{\columnwidth}{p{2cm} p{5.7cm}}
%     \toprule
    
%     \textbf{Data Type} & \textbf{Description} \\ \midrule
%     Rally breakdown & Time ranges (start and end), player who serves, and winning side  for all rallies in the match, manually annotated. \\ \hline
%     Shot breakdown  & Timestamps and the hitter of each shot, obtained from running MonoTrack~\cite{liu-2022} with minor manual clean-up. \\ \hline
%      3D shot & 3D trajectories and velocity for all shots from running MonoTrack~\cite{liu-2022}. \\ \hline
%     3D player poses & 3D player poses from running CLIFF~\cite{li-2022} on rally videos.\\ \hline
%     Shot tendency (offensive or defensive)  & Shot tendency approximated by the shuttle's velocity vector when passing the net, i.e., defensive when 
%     % the velocity vector drifts 
%     upward (away from the ground) and offensive when downward.
%     % (it always passes the net unless it is the last shot and one side made a mistake)
%     \\
% 	\bottomrule
% \end{tabularx}
% % \vspace{-6mm}
% \end{table}
% }



%For VIRD to support the goals and tasks outlined, the first step is to parse the match videos -- preferably in an automatic pipeline -- in order to obtain match-level and rally-level statistics, and useful spatial data. 
%Fortunately, several previous work in computer vision have already laid the foundation for what we want. 
%Specifically, MonoTrack~\cite{liu-2022} can predict court position, player poses, detect shots, and reconstruct 3D trajectories from monocular badminton videos for a rally; and CLIFF~\cite{li-2022} can predict smooth 3D player poses from monocular videos. Our data preprocessing pipeline is built on these two work. 
%We outline the important video-derived data we use in VIRD with a short description of how they are computed in Table~\ref{tab:data}.

% \begin{itemize}
%     \item Time ranges (start and end) for all the rallies in a video. We manually annotate this information for all our test videos. We also manually annotate which player serves, and which side wins the point in each rally.
%     \item Each shot in a given rally (in timestamp), and who hit it. This is from running MonoTrack~\cite{liu-2022} with minor manual clean-up.
%     \item 3D trajectories and velocity of each shot. We got this from running MonoTrack~\cite{liu-2022}.
%     \item 3D poses of the players. We got this from running CLIFF~\cite{li-2022}.
%     \item Shot tendency (offensive or defensive). We extract shot tendency by approximating the velocity vector of the shuttle when it passes the net (it always passes the net unless it is the last shot and one side made a mistake). If the velocity vector drifts upward (away from the ground), then it is defensive, otherwise it is offensive.
% \end{itemize}




% \begin{figure}[t!]
%   \centering
%   \includegraphics[width=\linewidth]{images/Summary.png}
%   \vspace{-6mm}
%   \caption{Main components in VIRD. Users use (a) and (b) to filter rallies listed in (c) based on the game and shot details. Static immersive visualizations of 3D shot data are shown in (d). When a shot or a rally is selected, dynamic game views are displayed on (e) and (f). 
%   }
%   \vspace{-4mm}
%   \label{fig:VIRD}
% \end{figure}


\subsection{VIRD Design}
To enable an ideal top-down match analysis, the VIRD interface features two modes: Summary Mode in a black background (Fig.~\ref{fig:teaser}-1) and Game Mode in a blue background (Fig.~\ref{fig:teaser}-2). The distinction between the two modes depends on whether the user is analyzing matches at a summary level (Summary) or exploring individual rallies (Game).
% 
% \noindent \textbf{Summary Mode}, as shown in Fig.~\ref{fig:teaser}-1, provides a high-level overview of the game statistics
% % (score breakdown, duration annotation, shot statistics, etc.), 
% and a rally filtering mechanism. 
% % based on users' interests. 
% This directly supports user needs in quickly summarizing a game, and drilling into details on demand (\textbf{G1} and \textbf{G2}).
% % 
% \noindent \textbf{Game Mode}, as shown in Fig.~\ref{fig:teaser}-2, provides a real-time, 3D reconstructed rally playback with dynamic shot trajectories and player poses. This allows users to investigate and interact with the data in context (\textbf{G2} and \textbf{G3}). 




% VR interface
%As shown in Fig.~\ref{fig:teaser}, the VR interface consists of two modes, a Summary Mode in black background (Fig.~\ref{fig:teaser}-1) and a Game Mode in blue background (Fig.~\ref{fig:teaser}-2), where the distinction between the two modes depends on whether the user is analyzing matches at a summary level (Summary) or delving into individual rally (Game).
%% 
%Summary Mode provides an overview of the match \textbf{(G1)} and guides the focus of the analysis by filtering and linking the static stats to the rally video \textbf{(G2)}. Game Mode presents 3D reconstructed game with dynamic shot trajectories and player pose along with 2D rally video \textbf{(G2 \& G3)}.



% Six main components of VIRD are shown in Fig.~\ref{fig:VIRD}. 
% \textit{Match Summary} (a)  provides an overview of the match and game statistics. 
% \textit{Shot Filter} (b) provides shot-level summary and allow filter shots by players, shot outcomes, and shot locations. 
% \textit{Rally Menu} (c) shows the list of filtered rallies with rally-level data, including length and score. 
% \textit{Virtual Court} (d) shows a 1-to-1 scale badminton court, where situated visualizations of 3D data and game views are projected, including shot arcs, heatmap, dynamic shot trajectory, and player poses. 
% \textit{Video View} (e) displays the original video footage of the selected shot or rally.
% \textit{3D Game View} (f) plays the reconstructed 3D game in sync with the video.
% % 
% Summary Mode always presents (a) to (d), and will show (e) and (f) when the user chooses a shot for preview; Game Mode presents (b) to (f) to show details of the selected rally with access to other similar rallies.
% 

Below, we described the detailed design of VIRD components and interaction between Summary and Game Mode to satisfy six analytic tasks. 
Descriptions are based on 2022 BWF World Championship match between Marin and Yamaguchi~\cite{match_marin_yamaguchi} (M2) used in case studies. 

\subsubsection{Visual Components}
\label{sec:visual_components}

\para{1) Statistical summary and filtering (T1, T2).}
In order to identify rallies of interest, experts need to break down the match and examine the statistics of games and rallies.  
We designed Match Summary and Shot Filter to support experts getting necessary metadata and filtering data in Summary Mode.
% , such as selecting all winner shots by Marin in Game 1. 



\setlength{\intextsep}{0pt}%
\begin{wrapfigure}{L}{0.23\textwidth}
	\centering
	\includegraphics[width=0.23\textwidth]{images/componentA.png}
	 \vspace{-8mm}
	\caption{Match Summary}
	 % \vspace{-2mm}
	\label{fig:match_summary}
\end{wrapfigure}

 % Match Summary 
With Match Summary, users can see the match's duration, rally count, average shot count per rally, the winner, and the scores of each game (T1). These statistics are essential to overview the pace and intensity of the match. 
A user can select the game and rallies won by a player from the game selector, e.g., 17 rallies won by Marin in G1. Similar statistics for the selected game are displayed below the game selector. 
Game 3 is split into two halves by default, as players switch sides at midpoint (when the leading side reaches 11 points) and therefore spatial data cannot be displayed on the same side of the court.
These metadata help experts identify games that were more challenging or outstanding for deeper analysis.
In addition, users can `split' a game into first and second half, similar to Game 3. This design was to provide finer granularity of the game. In the formative study, we found that sometimes experts would analyze each half separately, as players can receive coaching advice in a short break at the midpoint of each game. 

% Shot Filter

\FloatBarrier
\begin{wrapfigure}{R}{0.3\textwidth}
	\centering
	\includegraphics[width=0.3\textwidth]{images/componentB.png}
	 \vspace{-8mm}
	\caption{Shot Filter}
	 % \vspace{-2mm}
	\label{fig:shot_filter}
\end{wrapfigure}
Once the game is selected, Shot Filter allows users to specify the shot they want to analyze based on players and shot attributes, such as winners and errors (T2). According to the coaches in our user testing, this feature was considered extremely valuable as it provides an immediate comparison between the players. 
 
For example, among 17 rallies Marin scored, 9 points were due to Marin's winners while 8 were due to Yamaguchi's errors,
which tells a very different story if Marin had 17 winners. 
Further, a user can overview the shot distribution on the heat map and filter shots by areas, e.g., select the purple 56\% grid to filter Marin's winner shots hit from the back right. The darker color indicates more shots are \textit{from} (purple) or \textit{to} (orange) the area.
% 
The color schemes was considered helpful by experts to recognize hot spots or shot tendency between games or players, e.g. compare two players' heat map of winner shots.  


% Combining Match Summary and Shot Filter, the user can filter rallies based on game, players and shot attributes
% , which supports them focusing on rallies of interest. 
% All interactions are supported through VR controller's pointer and trigger button.
% Next, we discussed features that support detailed insight generation and verification across rallies.

% This feature fulfills the analysis tasks T2 and T3.

\para{2) Analyze statistical and spatial shot attributes (T3, T4).}
To help users identify shot patterns before diving into game details, we designed Rally Menu and Situated Visualizations to support immersive shot analysis within its game contexts in Summary Mode.

% Rally Menu
 \vspace{2mm}
\FloatBarrier
\begin{wrapfigure}{R}{0.18\textwidth}
	\centering
	\includegraphics[width=0.18\textwidth]{images/ComponentC.png}
	 \vspace{-6mm}
	\caption{Rally Menu}
	\label{fig:rally_menu}
\end{wrapfigure}
Rally Menu provides an overview of shot count and scoring cadence among the rallies of interest (T3). 
Each rally is presented on a rally item with score and length information in the scrollable menu. Short rallies (less than 10 shots) are highlighted in red to allow special focus based on coaches' requirements. For example, a user can tell the tempo of the game from the number of short rallies (4 out of 9) and the variation of shot counts between these rallies won by Marin. This overview of rally statistics supports finding patterns across rallies of interest.



% Situated Vis
\FloatBarrier
\begin{wrapfigure}{R}{0.25\textwidth}
	\centering
	\includegraphics[width=0.25\textwidth]{images/componentD.png}
	 \vspace{-6mm}
	\caption{Situated Visualizations}
	 % \vspace{-2mm}
	\label{fig:virtual_court}
\end{wrapfigure}
Based on the applied filters, 3D shot arcs and heatmap of the filter shots (e.g., all winners by Marin in Game 1) are visualized in-situ on the 1-to-1 virtual court.
The shots are color-coded based on the outcome (red for errors, green for winners, and white for all other shots). 
Upon interacting with the individual shot arcs, the shuttle's dynamic trajectory will be displayed in real-time (details in Sec.~\ref{sec:interaction}). 
The situated visualizations enable the user to derive insights into shots' spatial attributes (i.e., arc shapes, distributions). Experts use this design to quickly observe insights from shots across multiple rallies.

\para{3) Investigate game details of shot and rally (T5, T6).}
\FloatBarrier
\begin{wrapfigure}{R}{0.17\textwidth}
	\centering
	\includegraphics[width=0.17\textwidth]{images/componentE.png}
	 \vspace{-6mm}
	\caption{Game View}
	 % \vspace{-2mm}
	\label{fig:game_vieiw}
\end{wrapfigure}
Once some patterns are observed, it is necessary for experts to investigate actual game details to verify insights and investigate root causes. The user can preview the game moments of the chosen shot in Summary Mode, or delve into the entire rally in Game Mode.

Game View displays a 3D reconstructed game view simultaneously with the video to support a deeper investigation of the game details (T5). 3D game view presents the dynamic movement of shots and players to allow accurate spatial perception and flexible viewing angles. 

Upon examining the exact game moment of the chosen shot, the user can expand the analysis to the entire rally from the Game View or to other rallies containing similar shots from the Rally Menu (T6). 

% 
% Fig.~\ref{fig:Interaction}-2 shows the user interaction of linking from a shot in Summary Mode to the rally in Game Mode. 



% The user can select `View Match' from the hovered shot preview in Summary Mode (Fig.~\ref{fig:Interaction}-1) to watch the entire rally in Game Mode (Fig.~\ref{fig:Interaction}-2).

% 


\subsubsection{User Interaction}
\label{sec:interaction}
Users interact with VIRD interface and visualizations using VR controllers.
% 
Each shot can be hovered to select, which will link to the game context of the shot (Fig.~\ref{fig:Interaction}-1) in Summary Mode, showing Game View that contains 3D dynamic shot trajectory and player poses, and the same shot duration in the video.
This interaction allows users to instantly review the game moment of each shot in the filtered group (e.g., all winner shots) to obtain the context of 3D data. 
To navigate to the Game Mode (Fig.~\ref{fig:Interaction}-2), the users can select \textit{``View Match''} from the Game View of the hovered shot, or select a rally from the Rally Menu.
Furthermore, the user can directly hover over a shot arc in the rally (Fig.~\ref{fig:Interaction}-3) to play the video from the desired game moment.
This feature allows users to replay a specific shot or shot sequence easily.

Meanwhile, users can flexibly navigate the virtual court, by using a thumb stick or physically moving around, to obtain an accurate spatial and temporal perception of 3D data (Fig.~\ref{fig:Interaction}-3).
% 
VR environment also offers flexible viewpoints to analyze the 3D game from different perspectives, such as the first-person player view (Fig.~\ref{fig:Interaction}-4). 
% using shot start/end points on the ground to compare player coverage.


% In Game Mode, the shot arcs and foot positions of all shots in the selected rally are shown.

% When a shot or a rally is selected, \textbf{(e) Video View} displays the original video footage of the selected shot in repeat or the entire rally. \textbf{(f) 3D Game View} will play in sync with the video on the virtual court.
 % Rally Menu shows the list of rallies based on the Match Summary and Shot Filter criteria. Each rally is presented in a rally item card in the scrollable menu with score and length information. A user can select a rally to view the entire rally in Game Mode. The number of short rallies (less than 10 shots, based on formative study) is highlighted in red to allow special focus based on coaches' requirements.
% This feature supports T2, T4 and T5.


% ===========================

% \noindent
% \textbf{(a) Match Summary} provides an overview of the match and game statistics. At the top, a user can see the match's duration, the number of rallies, average shot count per rally, and the winner. A user can select the game and rallies won by a player for further analysis (e.g., 17 rallies won by Marin in G1 were selected in Fig.~\ref{fig:VIRD}a). Similar to the match statistics, duration and rally stats for the selected game are displayed below the game selector.
% This feature fulfills the analysis tasks T1 and T2.

%  \noindent
% \textbf{(b) Shot Filter} allows users to specify the shot they want to analyze based on players, shot outcome (errors, winners, or all shots), and shot locations (six areas on each side). Further, a user can use the shot heatmap to filter shots by areas (e.g., a user can select the purple 56\% grid to filter Marin's winner shots hit from the back right). The total number of filtered shots is shown to the right of the location filter. 
% Combining Match Summary and Shot Filter, the user can filter rallies based on game, players and shots, which supports them in finding rallies of interest.
% This feature fulfills the analysis tasks T2 and T3.
 
% \noindent
% \textbf{(c) Rally Menu} shows the list of rallies based on the Match Summary and Shot Filter criteria. Each rally is presented in a rally item card in the scrollable menu with score and length information. A user can select a rally to view the entire rally in Game Mode. The number of short rallies (less than 10 shots, based on formative study) is highlighted in red to allow special focus based on coaches' requirements.
% This feature supports T2, T4 and T5.
% % \jui{Is 10 justifiable from interview? I would justify more here.}

% \noindent
% \textbf{(d) Virtual Court} presents immersive visualizations for 3D data. In Summary Mode, a user can see the shot arcs, player's foot positions, and shot heat map projected onto the virtual court based on the selection in Shot Filter. The shots are color-coded based on the outcome (red for errors, green for winners, and white for all other shots). Each shot is interactable with the VR controller and will link to a video preview of the hovered shot. Details on the interaction are described in Sec.~\ref{sec:interaction}. In Game Mode, the shot arcs and foot positions of all shots in the selected rally are shown.
% When a shot or a rally is selected, \textbf{(e) Video View} displays the original video footage of the selected shot in repeat or the entire rally. \textbf{(f) 3D Game View} will play in sync with the video on the virtual court.
% These views collectively support T2, T4 and T5.



\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{images/Interaction.png}
  \vspace{-6mm}
  \caption{VIRD Interaction. 
  Users directly point at visualization to 1) preview a hovered shot and 2) link to the entire rally. They can use a thumb stick to 3) move flexibly in VR and 4) change viewing angle.}
  \vspace{-6mm}
  \label{fig:Interaction}
\end{figure}




% \subsection{Interaction}
% \label{sec:interaction}
% Both VR controllers to interact with VIRD are rendered as virtual hands, as shown in Fig.~\ref{fig:Interaction}-1-1. %, with the shape of hands, are used to interact with VIRD, 
% The left controller is used to point at a shot arc to trigger a shot preview in Summary Mode. When a shot is hovered, the left controller will provide a haptic feedback and both (e) Video View and (f) 3D Game View will be displayed while other shot arcs in (d) will be hidden. When the user hovers on the same shot again or presses on the reset button, the shot will be deselected with another haptic feedback, with the view reset to (d). The same interaction applies to Game Mode, with the difference that hovering a shot will repeat the shot in the rally video and deselecting will resume playback of the rest of the rally.
% % 
% The right controller is used to interact with all the buttons on the panels (a-c) to apply filters and select rally of interest. The thumb stick on the right controller allows the user to move freely in the horizontal direction. As shown in Fig.~\ref{fig:Interaction}-1, the user can change viewpoint flexibly to analyze the 3D visualizations or experience the game from the first-person view on the virtual court.

% Fig.~\ref{fig:Interaction}-2 shows the user interaction of linking from a shot in Summary Mode to the rally in Game Mode. For example, the user sets the Shot Filter with the right controller to view all error shots by \textit{Top} player. Then, the user points at an error shot to preview the shot in video with the left controller. Finally, the user selects from Rally Menu with the right controller to watch the entire rally in Game Mode.


\subsection{Design Iterations}
\label{sec:design_iteration}
We conducted three rounds of user testing throughout the design process. Three active high-performance badminton coaches in US were involved  (C1-C3; M=3; Age: 40-60), who were former players on the US, Malaysia, and Nepal badminton national teams, respectively. 
They have coaching experiences ranging from 15 to over 30 years. C1 had participated in our formative study while C2 and C3 were newly introduced at the design iteration stage.
Given the challenges in accessing domain experts, we adopted a progressive approach wherein each coach evaluated our prototype at various design stages, focusing on distinct aspects. 
We tested VIRD on the match of 2020 BWF World Tour Finals of Women Single between Tai and Marin~\cite{match_tai_marin}.

\noindent
\textbf{Round 1. User flow and data analysis.} The first testing was conducted on the initial prototype with C1, where we elicited the coach's feedback on the overall analysis approach and the shot filtering features.
The coach appreciated the top-down approach and interactive analysis process with immediate access to all match data and videos.
On top of the existing summary data and filters, he suggested showing winner and error shots separately to support an immediate comparison of the shot patterns.
Further, we designed two interaction methods to apply Shot Location Filter,  1) select buttons on the Shot Filter panel and 2) physically move to the desired area on the virtual court. However, the coach felt 1) is more useful as moving around the court to filter shots during the analysis would be tedious and distracting.

\noindent
\textbf{Round 2. Interaction with the visualization and interface.} The second testing was run a month later with C2, with a focus on the interaction of linking the static data to the dynamic trajectories and videos. We showed the dynamic bird trajectory of a hovered shot arc, but to view the original rally video the user had to scroll through and select from the Rally Menu.
The coach suggested augmenting the preview of the selected shot arc with the video, as \textit{``it takes time to find the video part of it right now''}.
He also emphasized the importance of pinpointing on the cause of the outcome during coaching. It is not enough to see where an error shot occurred in general, but to let the player see the shot sequence and player movement that lead to the outcome. 
Therefore, we implemented shot-to-rally interaction (Fig.~\ref{fig:Interaction}-1 to 2) to support coaches effectively look into specific rally where the error/winner occurs for detailed analysis into root cause. 

\noindent
\textbf{Round 3. Immersive 3D visualization.} We conducted the third test two months later with C3 on the usefulness of immersive visualizations. The coach was able to preview each group of filtered shots (e.g., winners) efficiently and interpreted the shot types from the 3D shot arcs to answer his coaching question, like \textit{``What are the shots Tai used to win?''- 1 cross drop [shot], 2 smash [shots], 1 block [shot]}. 
He also valued the color usage in the visualizations to tell the shot percentage on the heat map and highlight winner and error shots.
However, since 3D player poses were not implemented at the moment, we found all coaches still mainly watch the video view to analyze the rally as player movement is critical in finding the root cause,  e.g., \textit{``You hit the shot and it was a winning rally, why? Because the opponent wasn’t there yet''} (C2).
Both C2 and C3 mentioned the inclusion of player poses to enhance the usefulness and engagement of the 3D game view. Therefore, we worked on player pose estimation after the third user testing.

During the user testing, we also elicited coaches' feedback on VR environment.
% as all of them were first-time VR users. 
They agreed VR provides additional benefits in analyzing a match video, such as immediate access to all relevant information, flexible viewpoints, and an interactive approach. For instance, C1 commented \textit{``it was very helpful to see the video and the bird going with the trajectory at the same time.''}
% \textit{``when I put the headset on I already have information that I may need without even having to watch the video''} \jui{this is vague. what did D1 mean?}. 
C2 moved to the bottom left of the court while watching the 3D game view because \textit{``this is where I sit as a coach''}. C3 shared that the interaction to select a shot and link to the actual match video is very helpful as \textit{``it’s important to know how the player put the pressure and create a situation [in the game]''}.

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

